Stylos: Multi-View 3D Stylization with Single-Forward Gaussian Splatting

We present Stylos, a single-forward 3D Gaussian framework for 3D style transfer that operates on unposed content, from a single image to a multi-view collection, conditioned on a separate reference style image. Stylos synthesizes a stylized 3D Gaussian scene without per-scene optimization or precomputed poses, achieving geometry-aware, view-consistent stylization that generalizes to unseen categories, scenes, and styles. At its core, Stylos adopts a Transformer backbone with two pathways: geometry predictions retain self-attention to preserve geometric fidelity, while style is injected via global cross-attention to enforce visual consistency across views. With the addition of a voxel-based 3D style loss that aligns aggregated scene features to style statistics, Stylos enforces view-consistent stylization while preserving geometry. Experiments across multiple datasets demonstrate that Stylos delivers high-quality zero-shot stylization, highlighting the effectiveness of global style-content coupling, the proposed 3D style loss, and the scalability of our framework from single view to large-scale multi-view settings. Our codes are available at https://github.com/HanzhouLiu/Stylos.

==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/sections/acknowledgement.tex <==
\section{Acknowledgement}
% Acknowledgements for Delta and DeltaAI HPC
This research used both the DeltaAI advanced computing and data resource, which is supported by the National Science Foundation (award OAC 2320345) and the State of Illinois, and the Delta advanced computing and data resource which is supported by the National Science Foundation (award OAC 2005572) and the State of Illinois. Delta and DeltaAI are joint efforts of the University of Illinois Urbana-Champaign and its National Center for Supercomputing Applications. The allocations on Delta and DeltaAI [allocation number CIS250529] were made by the Advanced Cyberinfrastructure Coordination Ecosystem: Services \& Support (ACCESS) program, which is supported by National Science Foundation grants \#2138259, \#2138286, \#2138307, \#2137603, and \#2138296.

==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/sections/conclusion.tex <==
\section{Conclusion}
In this work, we propose Stylos, 
a feed-forward method for 3D stylization.
\
By keeping geometry predictions on the self-attentive backbone path 
and conditioning appearance via global CrossBlocks on the style path, 
together with a voxel-space 3D style loss that aggregates multi-view features, Stylos achieves geometry-aware and view-consistent stylization. 
\
Our ablations show that the global CrossBlock for style injection better preserves geometric details than alternative style-content fusion modules.
\
Extensive experiments across category-level and large-scale scene datasets demonstrate the generalization ability of our approach,
achieving aesthetically pleasing stylization with strong cross-view consistency.
\
In the future, we aim to scale Stylos to support higher-resolution inputs while improving efficiency, paving the way for practical 3D content creation.


==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/sections/experiment.tex <==
\section{Experiment}
\label{sec:exp}
\textbf{Datasets.}
We evaluate cross-category generalization on the CO3D~\citep{reizenstein2021common} dataset by training on 17 categories and testing on 3 held-out ones, 
and cross-scene generalization by training on the full DL3DV-10K~\citep{ling2024dl3dv} and testing on Tanks \& Temples~\citep{knapitsch2017tanks}. 
Style images are provided by WikiArt~\citep{wikiart} and DELAUNAY~\citep{gontier2023delaunay}, with 50 diverse style images reserved as unseen styles that are never used during training.

\textbf{Baselines.}
We compare \textbf{\textit{Stylos}} with recent 3D stylization models. The baselines include, (1) a per-scene training and zero-shot method StyleGaussian~\citep{liu2024stylegaussian}, (2) per-scene and per-style optimization approaches G-Style~\citep{kovacs2024gstyle}, StylizedGS~\citep{zhang2025stylizedgs}, and SGSST~\citep{galerne2025sgsst}, and (3) the closest related work Styl3R~\citep{wang2025styl3r}.

\textbf{Evaluation Metrics.}
Our evaluation covers three aspects. 
(1) To assess geometry reconstruction in the style-free setting, we report \emph{PSNR}, \emph{SSIM}, and \emph{LPIPS}~\citep{zhang2018unreasonable} 
between content views and predictions, conditioned on the original first frame of each scene as the style input. 
(2) To measure stylization consistency, following prior work~\citep{chiang2022stylizing}, 
we compute \emph{LPIPS} and \emph{RMSE} in both short-range and long-range settings. 
(3) To further evaluate stylization quality, we report \emph{ArtScore}~\citep{chen2024learning}, a recent metric specifically designed for reference-free evaluation of artness in generated images, 
and \emph{ArtFID}~\citep{wright2022artfid, chung2024style}.
%(consecutive frames $t$ and $t{-}1$) (distant frames $t$ and $t{-}7$)

\subsection{Ablation Study}
In this section, we analyze the impact of each design choice on the CO3D dataset. 
To ensure fairness, all variants are trained with identical configurations in each experimental round. 

% ########## Table 1 ##########
\input{iclr2026/tables/abl_frame_global}

% ########## Figure 2 ##########
\begin{figure*}[tb]
  \centering
  % left, bottom, right, top
  \includegraphics[width=0.98\linewidth, trim = 0.22cm 11.7cm 11.7cm 0.22cm]{iclr2026/figures/abl_attn.pdf}
  %\fbox{\includegraphics[width=0.98\linewidth, trim = 0.22cm 11.7cm 11.7cm 0.22cm]{iclr2026/figures/abl_attn.pdf}}

  \caption{CO3D pizza scene comparing different CrossBlock designs.}
  \label{fig:abl_attn}
\end{figure*}

\textbf{Discussions about CrossBlock Designs.}
Take the pizza scene for example. 
Table~\ref{tab:frame_global} shows that the baseline method, combining Frame and Global CrossBlock, yields a PSNR of 19.78 dB and LPIPS of 0.3326.
The frame variant produces slightly lower PSNR and higher LPIPS. 
By contrast, applying the Global CrossBlock significantly boosts the PSNR value by 0.79 dB and achieves consistently improved metrics. 
Qualitative comparisons in Fig.~\ref{fig:abl_attn} highlight these differences. 
Frame CrossBlock produces a poorly defined crust with noticeable artifacts, 
the hybrid variant recovers part of the structure but leaves the box edges blurred, 
while Global CrossBlock delivers the most faithful result, with clear toppings and a well-preserved crust boundary. 
\begin{figure*}[th]
  \centering
  % left, bottom, right, top
  \includegraphics[width=0.98\linewidth, trim = 0.22cm 0.3cm 0.8cm 0.32cm]{iclr2026/figures/StyleOG_loss_comparison.pdf}
  %\fbox{\includegraphics[width=0.98\linewidth, trim = 0.22cm 0.3cm 0.8cm 0.32cm]{iclr2026/figures/StyleOG_loss_comparison.pdf}}

  \caption{Comparison of style losses on unseen donut, skateboard, and pizza scenes from the CO3D dataset. Both scene and 3D style losses yield cleaner stylized textures compared to image-level matching, while the 3D loss further conveys a stronger sense of 3D geometry. We encourage readers to Appendix Fig.~\ref{fig:apdx_loss_comparisons_p1}-\ref{fig:apdx_loss_comparisons_p3} for more visual comparisons under varing scenes and styles.}\label{fig:abl_loss}
\end{figure*}

%\input{iclr2026/tables/abl_losses}
\input{iclr2026/tables/abl_losses_final} 

\textbf{Image vs. Scene vs. 3D Style Losses.}
As shown in Table~\ref{tab:style_loss}, both scene-level and 3D style losses clearly outperform the image-level baseline in terms of artistic quality. Overall, the 3D losses exhibit superior and more stable consistency performance.
These results indicate that enforcing style consistency in a voxel-level yields more coherent stylized textures across views. 
We observe that the image-level supervision may fail to transfer style.
For example, in Fig.~\ref{fig:abl_loss}, the donut surface is not well synthesized with the expected style, 
whereas the scene and 3D losses successfully apply the target style. 
The 3D style loss produces sharper boundaries and a stronger sense of 3D geometry, as observed in the skateboard and pizza examples, leading to the most coherent multi-view stylization.  
We release these model weights to support reproducibility and further analysis.

\textbf{From a Single View to Dozens of Views.}
%We further investigate the effect of view scaling on an unseen outdoor scene (Lighthouse from Tanks and Temples) with up to 64 frames and 10 style references. 
While Stylos can process up to dozens (even hundreds) of views, we observe a gradual decrease in visual quality once the number of views per batch (denoted as “\# views / batch”) exceeds 32. 
As shown in Fig.~\ref{fig:views}, very small batches (1 view) fail to synthesize parts of the scene like the bench, 
while overly large batches (64 views) introduce edge artifacts on the tall building, 
potentially due to the gap from our training settings (no more than 24 views).
Additionally, we provide~\ref{appendix:efficiency} Fig.~\ref{fig:scaling} to show the efficiency trend with respect to the number of views. 
%due to unstable Gaussian representations and the gap from training settings (no more than 24 views).
%According to Fig.~\ref{fig:scaling}, increasing \# views / batch increases per-batch runtime as more inputs are processed in parallel,  while GPU memory usage grows almost linearly.
\begin{figure*}[tb]
  \centering
  % left, bottom, right, top
  \includegraphics[width=\linewidth]{iclr2026/figures/StyleOG_view_comparison.pdf}
  %\fbox{\includegraphics[width=0.98\linewidth, trim = 0.25cm 12.9cm 6.9cm 0.28cm]{iclr2026/figures/views.pdf}}
  \caption{Effect of varying \# views / batch on the Lighthouse scene from Tanks and Temples.}\label{fig:views}
\end{figure*}

\input{iclr2026/tables/consistency}

\subsection{Comparison with State-of-the-Art}\label{sec:sota}
To retrain StyleGaussian~\citep{liu2024stylegaussian}, G-Style~\citep{kovacs2024gstyle}, StylizedGS~\citep{zhang2025stylizedgs}, and SGSST~\citep{galerne2025sgsst}, we strictly follow their released codes.
Since the pretrained-weights of StyleGaussian~\citep{liu2024stylegaussian} and Styl3R~\citep{wang2025styl3r} are publicly available, we use them to generate the visual results.
Stylos is trained once on DL3DV~\citep{ling2024dl3dv}, and tested in a zero-shot manner without prior knowledge of either the scenes or styles.

\textbf{Quantitative Evaluation.}
As shown in Table~\ref{tab:consistency}, Stylos achieves strong and stable consistency scores, ranking the first across all consistency metrics and all four scenes. This indicates that Stylos provides markedly improved cross-view stylization consistency.
\
Furthermore, Table~\ref{tab:artscore} shows that Stylos attains either the best or second-best artistic metric values, as rated by ArtScore and ArtFID, on all four Tanks and Temples scenes~\citep{knapitsch2017tanks}, while maintaining the fastest stylization speed.
\
Overall, Stylos demonstrates a favorable balance between visual quality, consistency, and efficiency, suggesting its potential for practical real-time 3D stylization.

\input{iclr2026/tables/artscore_artfid_time}

\begin{figure*}[tb]
  \centering
  % left, bottom, right, top
  \includegraphics[width=0.98\linewidth, trim = 0.22cm 0.3cm 0.8cm 0.32cm]{iclr2026/figures/sota_comparison_reorder.pdf}
  %\fbox{\includegraphics[width=0.98\linewidth, trim = 0.22cm 0.3cm 0.8cm 0.32cm]{iclr2026/figures/StyleOG_sota_comparison.pdf}}

  \caption{Visual comparisons between \textbf{\textit{Stylos}} and recent 3D stylization approaches. \textbf{\textit{Stylos}} successfully transfers diverse artistic styles to the scenes while preserving fine structural details.}\label{fig:visual_comparisons_w_sota}

\end{figure*}

\textbf{Qualitative Evaluation.}
Taking the truck scene with the \textit{desert-town} style (yellow foreground objects with blue backgrounds) in Fig.~\ref{fig:visual_comparisons_w_sota} as an example, we observe that nearlly all existing approaches could reasonably produce structured results. However, their differences are discussed as follows. The zero-shot method StyleGaussian fail to generate color-consistent scenes, several portions of the truck retain undesired color blocks. Per-scene and per-style fitting approaches such as G-Style, StylizedGS, and SGSST often fail to achieve complete style transfer, the truck door remaining predominantly blue instead of adopting the target yellow hue. The other feedforward solution Styl3R similarly struggles to propagate the correct yellow color throughout the truck.
\
In contrast, Stylos successfully renders the truck in coherent yellow while preserving clean geometry, and correctly assigns blue tones to the distant background regions, producing an appearance that closely resembles the intended desert-town aesthetic. These observations underscore the strength of Stylos in achieving both faithful style expression and robust 3D structural preservation.

\subsection{Evaluation of Multi-Style Blending and Stylization Control}
We validate the model’s controllable stylization capability through two interpolation experiments. First, by linearly interpolating between the embeddings of two distinct style images, we observe smooth, coherent transitions that demonstrate the model’s natural support for multi-style blending (see Fig.~\ref{fig:combined_interpolation}).
Second, because the model is trained to reconstruct the original appearance when the style image matches the content image, we interpolate between the reconstruction (content) embedding and a stylized embedding Fig.~\ref{fig:combined_interpolation}. This produces a continuous spectrum of outputs with gradually increasing stylization strength, confirming that our approach enables fine-grained, post-inference control over the content–style trade-off. Together, these results show that our method supports both multi-style fusion and adjustable stylization without any additional optimization.
\begin{figure*}[tb]
  \centering
  \includegraphics[width=\linewidth]{iclr2026/figures/1414_23_linear.jpg}
  \includegraphics[width=\linewidth]{iclr2026/figures/original_201_linear.jpg}
  \caption{Evaluation of multi-style blending and controllable stylization.
Top: interpolation between two style embeddings.
Bottom: interpolation between the content embedding and a style embedding.}
  \label{fig:combined_interpolation}
\end{figure*}

==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/sections/introduction.tex <==
\section{Introduction}
Image guided 3D stylization aims to preserve scene geometry and cross-view consistency while transferring the reference style. 
\
With the rise of immersive content, augmented and virtual reality,
demand for this capability is growing.
Nevertheless, achieving reliable 3D stylization remains challenging and continues to attract significant research attention~\citep{chen2025advances}.

Early attempts typically focus on 3D representations such as meshes, volumetric data, and point clouds~\citep{kato2018neural,liu2018paparazzi,kim2019transport,kim2020lagrangian,guo2021volumetric,cao2020psnet}.
The introduction of implicit neural radiance fields (NeRF)~\citep{mildenhall2020nerf}, enables higher-fidelity rendering, and subsequent works extended it to artistic stylization~\citep{zhang2022arf,huang2022stylizednerf,Nguyen2022SNeRF,bao2022sine,liu2023stylerf},
but typically require costly per-scene optimization, constraining their generalization to unseen scenes.
More recently, 3D Gaussian Splatting (3DGS) has emerged as a promising explicit representation that combines high reconstruction quality with real-time rendering efficiency~\citep{kerbl20233d}.
Stylization approaches built on 3DGS achieve efficient multi-view consistency~\citep{liu2024stylegaussian,mei2024regs,galerne2025sgsst}, yet still struggle to generalize beyond scene-specific training.

In contrast, we introduce \textbf{\textit{Stylos}} (meaning \textit{pens} in French), 
a single-forward framework for 3D style transfer that eliminates the need for per-scene optimization and precomputed camera parameters, 
and generalizes effectively to novel categories, scenes, and styles.
\
Stylos employs a shared Transformer backbone with two pathways: content and style images are projected into a shared feature space, where content retains self-attention for geometric reasoning, and style is injected via the CrossBlock modules that are primarily composed of a self-attention layer followed by cross-attention.
\
Geometry-related attributes, such as depth, camera intrinsics, and extrinsics,
are derived from backbone features, 
whereas style conditioning guides the prediction of color coefficients.
These outputs are estimated through prediction heads that serve as the interface between
feature space and the final Gaussian representation.
\
A representative style loss function in 2D style transfer is based on feature distribution alignment~\citep{li2017demystifying,huang2017arbitrary,jing2019neural,singh2021neural}, which operate on image-level statistics and do not explicitly enforce multi-view or structural consistency required for 3D stylization.
\
To address this, we explore alternative objectives and propose a voxel-level 3D style loss that aligns aggregated scene features with style statistics, providing stronger view-consistent stylization while preserving geometric fidelity.

We evaluate Stylos across different scenarios, including category-level transfer and cross-scene generalization. Our assessment spans challenging real-world benchmarks, where Stylos produces stylized renderings with high visual fidelity and consistent geometry, demonstrating robustness even in previously unseen environments.
Our main contributions are threefold:

\begin{itemize}
\item We propose a shared-backbone design with two pathways: geometry predictions retain self-attention for geometric reasoning, while style is injected through cross-attention.
\item We introduce a voxel-level 3D style loss that aligns aggregated scene features with style statistics, enforcing cross-view coherence and geometry-aware stylization.
\item We develop Stylos, a single-forward-pass pipeline for 3D style transfer from unposed inputs, scaling from a single to hundreds of views with a single style image, and achieving zero-shot generalization to unseen categories, scenes, and styles.
\end{itemize}




==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/sections/limitation.tex <==
\section{Limitation}
The main limitations of Stylos are provided as follows. (1) We observe that using a large CLIP weight may overemphasize semantic alignment at the expense of fine-grained texture details. Developing more principled strategies for multi-loss balancing could further improve stylization fidelity. (2) Stylos can process entire scenes with dozens (even hundreds) of input views, but its computation cost and latency increase correspondingly, as analyzed in Appendix~\ref{appendix:efficiency}. 

==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/sections/method.tex <==
\begin{figure*}[tb]
  \centering
  % left, bottom, right, top
  \includegraphics[width=\linewidth]{iclr2026/figures/arch_new.pdf}
  %\fbox{\includegraphics[width=\linewidth, trim = 0cm 0cm 0cm 0cm]{iclr2026/figures/arch_new.pdf}}

  \caption{{\bftab Architecture overview}. Given multi-view content inputs and a style reference, Stylos enables instant 3D stylization without scene-specific training or post-optimization. Its core CrossBlock module facilitates style injection by integrating a cross-attention layer between self-attention and MLP. The proposed 3D style loss matches voxelized 3D features with 2D style statistics.}\label{fig:arch}
\end{figure*}

\section{Method}\label{sec:method}

We propose \textbf{\textit{Stylos}}, a transformer-based framework for stylized 3D scene reconstruction.
Given a style reference image and one or more content views (also referred to as context views),
Stylos predicts a set of stylized 3D Gaussian primitives together with camera parameters,
enabling faithful reconstruction of the observed scene while transferring the desired style.
We first formulate the problem in Sec.~\ref{sec:problem}, 
then present the network architecture in Sec.~\ref{sec:architecture}, 
and finally detail our training strategy in Sec.~\ref{sec:training} and the used style loss in Sec.~\ref{sec:style_loss}.


\subsection{Problem Formulation}
\label{sec:problem}

We aim to disentangle geometry and style within a unified 3D scene representation. 
The input to Stylos consists of a set of $N$ context views 
$\{I_i\}_{i=1}^N$ of a scene, with $N \geq 1$ and 
$I_i \in \mathbb{R}^{H \times W \times 3}$, together with a single 
style reference image $S \in \mathbb{R}^{H \times W \times 3}$. 
The context views provide geometric cues, while the style image specifies 
the desired aesthetic. 

Formally, Stylos defines a conditional mapping,
\[
    f_\theta: (\{I_i\}_{i=1}^N,\, S) \;\mapsto\; \big(G,\, \{g_i\}_{i=1}^N \big),
    \label{eq:condmap}
\]
where the scene representation $G = \{(p_m,\, c_m)\}_{m=1}^M$ 
is parameterized by $M$ anisotropic 3D Gaussians. 
Each Gaussian has geometry attributes 
$p_m = (\mu_m,\, \alpha_m,\, r_m,\, s_m)$, comprising 
3D position $\mu_m \in \mathbb{R}^3$, 
opacity $\alpha \in \mathbb{R}^+$, 
orientation quaternion $r_m \in \mathbb{R}^4$, 
and anisotropic scale $s_m \in \mathbb{R}^3$, 
as well as a style-dependent color embedding 
$c_m \in \mathbb{R}^{3 \times (k+1)^2}$ 
represented with spherical harmonics of degree $k$. 
In addition, Stylos jointly predicts camera parameters 
$\{g_i \in \mathbb{R}^9\}_{i=1}^N$ for each input view, 
leveraging pose cues estimated by the VGGT backbone.%~\citep{wang2025vggt}.

\subsection{Network Architecture}
\label{sec:architecture}

%\textbf{Architecture Overview.} 
Stylos employs a geometry backbone that alternates frame-wise and global attention to process multiple input views and infer geometry-related parameters such as positions, scales, orientations, and opacities. 
To enable stylization, we introduce a dedicated conditioning branch, where the \emph{Style Aggregator} fuses content and style features through cross-attention and predicts style-aware color embeddings for each Gaussian. 
In this way, geometry remains derived solely from the backbone, while style representation is conditioned on the style reference. 
We next detail the geometric backbone in Sec.~\ref{sec:geom_backbone}, the style aggregation module in Sec.~\ref{sec:style_agg}, and the prediction heads in Sec.~\ref{sec:heads}. 
%providing a complete view of how Stylos disentangles geometry and style while jointly supporting pose estimation and stylization.


\subsubsection{Geometric Backbone}
\label{sec:geom_backbone}
The geometric backbone follows the alternating-attention design of 
VGGT~\citep{wang2025vggt}, which interleaves frame and global 
self-attention layers to capture both intra-frame structure and 
cross-view consistency. 
This component is kept unchanged to retain strong geometric reasoning, 
serving as the foundation on which we integrate style information.

%\subsubsection{Style Aggregator}
% \label{sec:style_agg}
% The Style Aggregator extends the geometric backbone by adapting its attention layers from self-attention to cross-attention. 
% Both content views and the style image are embedded with a shared patch encoder, ensuring that their tokens lie in a common feature space. 
% In this design, content tokens serve as queries while style tokens provide keys and values, 
% so that style information conditions the token representations later used for predicting Gaussian colors. 
% Geometry-related parameters, in contrast, are still predicted from the backbone pathway and remain unaffected by style conditioning.

% \textbf{Content--Style Coupling.} Let $\mathcal{Q}_{b,v} \in \mathbb{R}^{L_q \times C}$ denote the content tokens extracted from 
% the $v$-th view of the $b$-th sample, and let $\mathcal{KV}_{b} \in \mathbb{R}^{L_{kv} \times C}$ 
% denote the style tokens. We use $\mathrm{XAttn}(\mathcal{Q}, \mathcal{KV})$ to denote a standard 
% cross-attention operator that updates $\mathcal{Q}$ using $\mathcal{KV}$ as key--value pairs.
% Depending on how the query set is formed, we consider three content--style coupling mechanisms. 

% \textbf{(1) Frame cross attention.}
% Each view independently interacts with the style tokens,
% \begin{equation}
%     \widetilde{\mathcal{Q}}_{b,v}
%     =
%     \mathrm{XAttn}(\mathcal{Q}_{b,v},\, \mathcal{KV}_{b}).
%     \label{eq:frame_xattn}
% \end{equation}
% This preserves view-specific structure but does not propagate information across views.

% \textbf{(2) Global cross attention.}
% We first concatenate all views to obtain a global sequence $\mathcal{Q}_b^{\mathrm{global}} \in \mathbb{R}^{VL_{q} \times C}$ by $\mathcal{Q}_b^{\mathrm{global}}=\mathrm{Concat}_{v=1}^{V} \mathcal{Q}_{b,v}$, 
% and perform cross-attention,
% \begin{equation}
%     \widetilde{\mathcal{Q}}^{\mathrm{global}}_{b}
%     =
%     \mathrm{XAttn}(\mathcal{Q}^{\mathrm{global}}_{b},\, \mathcal{KV}_b).
%     \label{eq:global_xattn}
% \end{equation}
% We then reshape the updated tokens back to per-view tensors,
% $\widetilde{\mathcal{Q}}_{b,v}$, by splitting 
% $\widetilde{\mathcal{Q}}^{\mathrm{global}}_{b}$ along the sequence dimension.
% This cross attention enables long-range reasoning across views and the style.

% \textbf{(3) Hybird cross attention.}
% We first apply frame attention to refine each view independently as in Eq.~\ref{eq:frame_xattn},
% and then perform global attention by concatenating $\widehat{\mathcal{Q}}_{b,v}$ across views
% and applying the same cross-attention operator as in Eq.~\ref{eq:global_xattn}.
% This hierarchical coupling is expected to combine per-view refinement with multi-view aggregation.
% For completeness, we concatenate their outputs along the channel dimension to form the final token representation.



\subsubsection{Style Aggregator}
\label{sec:style_agg}
The Style Aggregator builds on the geometric backbone inherited from VGGT, which is composed of standard Transformer $\mathrm{Block}$ containing self-attention followed by feed-forward layers. To enable style conditioning, we replace this standard block with an adapted \textit{cross fusion block} ($\mathrm{CrossBlock}$), which inserts a cross-attention operation between the self-attention and MLP stages~\citep{deng2022stytr2}. In $\mathrm{CrossBlock}$, content tokens serve as queries ($\mathcal{Q}$) while style tokens provide keys and values ($\mathcal{KV}$). This structure allows the content representations to be refined by their own spatial context (via the preserved self-attention), while being explicitly conditioned on the target style (via the inserted cross-attention) before the final feed-forward projection.

\textbf{Cross Fusion Blocks.} Let $\mathcal{Q}_{b,v} \in \mathbb{R}^{L_q \times C}$ denote the content tokens extracted from 
the $v$-th view of the $b$-th sample, and let $\mathcal{KV}_{b} \in \mathbb{R}^{L_{kv} \times C}$ 
denote the style tokens. We use $\mathrm{CrossBlock}(\mathcal{Q}, \mathcal{KV})$ to denote our block operator 
that updates $\mathcal{Q}$ using $\mathcal{KV}$ as key--value pairs.
Depending on how the query set is formed, we consider two primary topological strategies.

\textbf{(1) Frame CrossBlock.}
Each view independently interacts with the style tokens,
\begin{equation}
    \widetilde{\mathcal{Q}}_{b,v}
    =
    \mathrm{CrossBlock}(\mathcal{Q}_{b,v},\, \mathcal{KV}_{b}).
    \label{eq:frame_xattn}
\end{equation}
Since the internal self-attention of the block operates only on $\mathcal{Q}_{b,v}$, this strategy preserves view-specific geometric structure but prevents information propagation between different views.

\textbf{(2) Global CrossBlock.}
We first concatenate all views to obtain a global sequence $\mathcal{Q}_b^{\mathrm{global}} \in \mathbb{R}^{VL_{q} \times C}$ by $\mathcal{Q}_b^{\mathrm{global}}=\mathrm{Concat}_{v=1}^{V} \mathcal{Q}_{b,v}$, 
and perform the block operation simultaneously,
\begin{equation}
    \widetilde{\mathcal{Q}}^{\mathrm{global}}_{b}
    =
    \mathrm{CrossBlock}(\mathcal{Q}^{\mathrm{global}}_{b},\, \mathcal{KV}_b).
    \label{eq:global_xattn}
\end{equation}
We then reshape the updated tokens back to per-view tensors,
$\widetilde{\mathcal{Q}}_{b,v}$, by splitting 
$\widetilde{\mathcal{Q}}^{\mathrm{global}}_{b}$ along the sequence dimension.
This approach enables long-range reasoning: the internal self-attention ensures multi-view geometric consistency, while the cross-attention broadcasts style information globally.

\textbf{(3) Hybrid CrossBlocks.}
We first apply Frame CrossBlock to refine each view independently as in Eq.~\ref{eq:frame_xattn},
and then perform Global CrossBlock by concatenating the resulting $\widehat{\mathcal{Q}}_{b,v}$ across views
and applying the same operator as in Eq.~\ref{eq:global_xattn}.
This hybrid design combines per-view refinement with multi-view aggregation.
We direct readers to the released codes for implementations.

\subsubsection{Prediction Heads}
\label{sec:heads}
To connect the geometric backbone and Style Aggregator with the Gaussian scene,
we introduce prediction heads that translate feature tokens into explicit parameters.
These heads serve as modular interfaces, keeping geometry and style distinct in feature space
while ensuring their integration in the final Gaussian representation.
We next describe the individual heads in detail.

\textbf{Geometry Head.}
Geometric backbone features are passed through a DPT-style regression head that outputs the Gaussian geometry parameters
$p_m = (\mu_m, s_m, r_m, \alpha_m)$, i.e., position, scale, orientation, and opacity (as defined in Sec.~\ref{sec:problem}).
By relying on this established design, structural predictions are derived from backbone features alone, without direct influence from style conditioning.

\textbf{Style Head.}
The outputs of the Style Aggregator are subsequently processed by a color head to predict the spherical-harmonic coefficients $c_m$ that define appearance.
This pathway injects style information directly into Gaussian colors while leaving the geometry parameters $p_m$ unaffected,
enabling the two factors to be recombined seamlessly at the Gaussian level.

\textbf{Auxiliary Heads, Adapter, and Voxelization.}
We employ the existing VGGT camera head to estimate camera intrinsics and extrinsics, 
and a depth head to predict scene geometry cues, 
which are unprojected into 3D anchors for Gaussian placement~\citep{kerbl20233d,ren2025octree}. 
A Gaussian adapter then consolidates geometry and style outputs into a unified set of primitives $\{(p_m, c_m)\}_{m=1}^M$ for differentiable rendering. 
Finally, to reduce redundancy and balance density, we follow the voxelization step introduced by AnySplat~\citep{jiang2025anysplat},
nearby points are clustered within a discretized 3D grid and fused using confidence-aware weighting. 
This operation depends only on the unprojected 3D points and features, and is independent of camera parameters.

\subsection{Training Strategy}
\label{sec:training}

We adopt a two-stage training strategy for structure-aware stylization. 

\textbf{Stage 1: Geometry Pretraining.}
We initialize the geometric backbone of Stylos with VGGT weights~\citep{wang2025vggt} and train the network end-to-end to learn geometry and photometric appearance. 
To avoid trivial identity mapping and improve robustness to color variations, 
one input view is randomly selected and color-jittered as the style reference.
A frozen VGGT teacher provides pose and depth supervision. 
The objective combines reconstruction and distillation,
\[
\mathcal{L}_{\text{stage1}} 
= \mathcal{L}_{\text{rec}} 
+ \lambda_{\text{distill}} \, \mathcal{L}_{\text{distill}}.
\]

\textbf{Stage 2: Stylization Fine-tuning.}
We freeze all geometry-related modules and only update the Style Aggregator and the color head. 
Following ArtFlow~\citep{an2021artflow}, we use feature-level style and content losses in VGG space, 
matching channel-wise statistics for style and feature activations for content. 
We further extend these objectives with a 3D voxel-space style loss for cross-view consistency, 
and add a CLIP-based loss for semantic alignment. 
A total variation (TV) regularizer is also included to suppress high-frequency artifacts and stabilize optimization. 
The total loss is,
\[
\mathcal{L}_{\text{stage2}} 
= \mathcal{L}_{\text{rec}} 
+ \lambda_{\text{style}} \, \mathcal{L}_{\text{style}}^{3D} 
+ \lambda_{\text{cnt}} \, \mathcal{L}_{\text{content}} 
+ \lambda_{\text{clip}} \, \mathcal{L}_{\text{clip}} 
+ \lambda_{\text{tv}} \, \mathcal{L}_{\text{TV}}.
\]
In our experiments, we set $\lambda_{\text{distill}} = 1.0$, and use $\{{\lambda_{\text{style}}, \lambda_{\text{cnt}}, \lambda_{\text{clip}}, \lambda_{\text{tv}}}\} = \{{1.0, 0.1, 1.0, 10.0}\}$%\footnote{Refer to our released code for the complete loss configuration details.}.

\subsection{Style Losses}
\label{sec:style_loss}

We denote by $\mathcal{R}^l_{b,v} \in \mathbb{R}^{C_l \times H_l \times W_l}$ the VGG feature map 
of the rendered image for the $b$-th scene and $v$-th view at layer $l$, 
and by $\mathcal{S}^l_b \in \mathbb{R}^{C_l \times H_l \times W_l}$ the feature map of the single style image. 
Building on the Batch
Normalization statistics method~\citep{li2017demystifying}, 
which interprets BN mean and variance as style descriptors, 
we progressively extend it matching beyond standard 2D settings. 
This progression starts from independent image-level matching, moves to multi-view feature aggregation that promotes global style coherence across views, and culminates in a voxel-space loss that directly constrains the fused 3D representation. Next, we formulate the three losses studied in this paper.

\textbf{Image-Level Style Loss.}
The simplest baseline aligns each rendered frame independently with the style reference, which encourages per-frame stylization but does not enforce multi-view consistency,
\begin{equation}
\mathcal{L}^{\mathrm{img}}_{\mathrm{sty}}
= \frac{1}{BV}\sum_{b=1}^B\sum_{v=1}^V\sum_{l=1}^{5}\alpha_l
\Bigl(\|\mu(\mathcal{R}^l_{b,v})-\mu(\mathcal{S}^l_b)\|_2^2+\|\sigma(\mathcal{R}^l_{b,s})-\sigma(\mathcal{S}^l_b)\|_2^2\Bigr),
\label{eq:img_loss}
\end{equation}
where $\alpha_l$ denotes the weight at each level $l$, $\mu$ is the mean and $\sigma$ is the standard deviation.

\textbf{Scene-Level Style Loss.}
To introduce consistency into multi-view 3D stylization, 
we concatenate the per-view features $\{\mathcal{R}^l_{b,v}\}_{v=1}^V$ 
along the spatial dimension to form $\widetilde{\mathcal{R}}^l_b$, 
and calculate statistics on this aggregated map. However, this method still operates in 2D feature space and is computed by,
\begin{equation}
\mathcal{L}^{\mathrm{scn}}_{\mathrm{sty}}
= \frac{1}{B}\sum_{b=1}^B\sum_{l=1}^{5}\alpha_l
\Bigl(\|\mu(\widetilde{\mathcal{R}}^l_b)-\mu(\mathcal{S}^l_b)\|_2^2+\|\sigma(\widetilde{\mathcal{R}}^l_b)-\sigma(\mathcal{S}^l_b)\|_2^2\Bigr).
\label{eq:scn_loss}
\end{equation}

\begin{algorithm}[tb]
\caption{3D Voxel-based AdaIN Style Loss}
\begin{algorithmic}[1]
\REQUIRE Rendered features $\mathcal{R}$, Style features $\mathcal{S}$, 3D points $\mathcal{P}$, Confidence $\mathcal{C}$, Valid mask $\mathcal{M}$
\ENSURE 3D style loss $\mathcal{L}_{sty}^{\text{3D}}$
\STATE Initialize $\mathcal{L}_{sty}^{3D} \leftarrow 0$
\FOR{$b = 1$ to $B$}
  \FOR{$l = 1$ to $5$}
    \STATE Resize $(\mathcal{C, M, P})$ to match the resolution of $\mathcal{R}^l_{b}$
    \STATE \textit{// Next, fuse all views into a single voxel grid}
    \STATE $\mathcal{G}_b^l \leftarrow \text{VoxelizeAndFuse}\left(
        \{\mathcal{R}^l_{b,v}\}_{v=1}^V,
        \{\mathcal{P}_{b,v}\}_{v=1}^V,
        \{\mathcal{C}_{b,v}\}_{v=1}^V,
        \{\mathcal{M}_{b,v}\}_{v=1}^V
    \right)$
    \STATE \textit{// Next, compute the BN statistics (mean and standard deviation) of two feature maps}
    \STATE $(\mu_g, \sigma_g) \leftarrow \text{MeanStd}(\mathcal{G}_b^l)$, 
    $(\mu_s, \sigma_s) \leftarrow \text{MeanStd}(\mathcal{S}_b^l)$
    \STATE $\mathcal{L}_{sty}^{3D} \leftarrow \mathcal{L}_{sty}^{3D} +
           \alpha_l\|\mu_g - \mu_s\|_2^2 + \alpha_l\|\sigma_g - \sigma_s\|_2^2$
  \ENDFOR
\ENDFOR
\STATE \textbf{return} $\mathcal{L}_{sty}^{3D} 
  = \lambda_{sty} \mathcal{L}_{sty}^{3D}$
\end{algorithmic}\label{alg:3d_loss}
\end{algorithm}

\textbf{Voxel-level 3D Style Loss.}
Finally, to further enforce multi-view consistency, we fuse multi-view features into a voxel grid using differentiable unprojection, 
where features from different views are accumulated into spatial bins of a discretized 3D volume. 
Let $\mathcal{G}^l_b$ denote the voxelized features for the $b$-th scene at layer $l$. 
We then compute style statistics directly in voxel space,
\begin{equation}
\mathcal{L}^{\mathrm{3D}}_{\mathrm{sty}}
= \frac{1}{B}\sum_{b=1}^B\sum_{l=1}^{5}\alpha_l
\Bigl(\|\mu(\mathcal{G}^l_b)-\mu(\mathcal{S}^l_b)\|_2^2+\|\sigma(\mathcal{G}^l_b)-\sigma(\mathcal{S}^l_b)\|_2^2\Bigr).
\label{eq:3d_loss}
\end{equation}
By operating on voxelized features, this loss explicitly encodes geometry and 
enforces style consistency across both views and the underlying 3D structure.
We provide pseudo codes in Algorithm~\ref{alg:3d_loss}.

==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/sections/related_work.tex <==
\section{Related Work}


\subsection{Single-Forward 3D Reconstruction}
% Most NeRF and 3DGS methods assume access to accurate camera pose, which introduces an implicit preprocessing step that conceals the significant time and logistical costs of large-scale, multi-view data acquisition and registration. To overcome these limitations,

Recent advances in 3D reconstruction have shifted from optimization-heavy pipelines to single-forward models that directly predict structure and camera parameters from raw images. Early CNN-based attempts such as \emph{DeMoN} \cite{ummenhofer2017demon}, \emph{DeepTAM} \cite{zhou2018deeptam} and \emph{DeepV2D} \cite{Teed2020DeepV2D:} demonstrate feasibility but fell short of classical methods. The transformer era brought large-scale models like DUSt3R \cite{wang2024dust3r} and its extension MASt3R \cite{leroy2024grounding}, which replaced multi-stage SfM pipelines with single-pass predictions of geometry and poses. While effective, these models require expensive post-processing and often struggle with alignment in complex multi-view settings. Subsequent works such as Spann3R \cite{wang2024spann3r},CUT3R \cite{wang2025continuous} and MUSt3R \cite{cabon2025must3r} reduced reliance on classical optimization by incorporating memory or parallelized attention but incurred high computational costs at the same time. More recently, VGGT \cite{wang2025vggt} introduced alternating-attention transformers for joint multi-view inference of depth, pose and pointmaps, which achieves more consistent and scalable resonctructions. In parallel, feed-forward Gaussian splatting methods like AnySplat \cite{jiang2025anysplat} demonstrate that end-to-end pipelines can jointly recover geometry, camera intrinsics and novel views directly from uncalibrated images. Our work is inspired by such methods and aims to extend them to 3D style transfer. 


\subsection{3D Style Transfer}
% 3D scene stylizing has attracted growing research efforts.
Early works have achieved impressive 3D scene style transfer results over diverse explicit representations such as mesh~\citep{kato2018neural,michel2022text2mesh,Hollein_2022_CVPR}, voxel~\citep{guo2021volumetric} and point cloud~\citep{huang2021learning,mu20223d,cao2020psnet}. However, the quality of their results is limited by the precision of the geometric reconstructions, which often leads to noticeable artifacts in complex real-world scenes. 

The advent of implicit neural representations like Neural Radiance Fields (NeRF)~\citep{mildenhall2020nerf} has provided a more visually compelling and geometry-consistent results for 3D scene stylization. \cite{Nguyen2022SNeRF} use individually stylized
images rendered from a pre-trained NeRF as targets, iteratively fine-tuning the model to align with the desired style in a view-consistent manner. \emph{ARF} \cite{zhang2022arf} 
follows a similar approach but employs a nearest neighbor matching loss on the features extracted from rendering
and style instead of a standard color loss.
%transfers artistic features from 2D style images to 3D scenes, treating stylization as an optimization problem within the NeRF framework. 
To allow for zero-shot style transfer,~\citep{chiang2022stylizing}frames 3D stylization as style injection into a NeRF scene via a hypernetwork, which maps a reference style image to scene-conditioned parameters. \emph{StylizedNeRF}~\citep{huang2022stylizednerf} jointly learns 2D and 3D stylization. \emph{StyleRF}~\citep{liu2023stylerf} then performs style transformation in the radiance-field feature space, improving geometry and supporting zero-shot transfer to new styles. Despite these advances, NeRF-based methods remain computationally expensive, the rendering speed is limited by their volumetric nature, which restrict their usability in real-time scenarios. 
%requiring dense posed inputs and lengthy per-scene optimization, which restrict their usability in interactive or casual scenarios. 
%StyleRF learns high level features in 3D space for fast zero-shot style transfer.

Recently, 3D Gaussian Splatting (3DGS) \cite{kerbl20233d} has emerged as a promising explicit yet efficient representation for stylization. Unlike NeRFs, 3DGS enables real-time rendering while maintaining high reconstruction quality. \emph{ReGS} \cite{mei2024regs} refines a pre-trained 3DGS to a single style using a texture-guided control mechanism. \emph{StyleGaussian}~\citep{liu2024stylegaussian} proposes an efficient feature rendering strategy capable of swiftly rendering high-dimensional VGG features. 
% avoid per-asset optimization by embedding VGG features into each Gaussian splat which are then modulated based on a target style image and decoded back to stylized colors. 
\emph{StylizedGS}~\citep{zhang2024stylizedgs} is an optimization-based method that extends \emph{ARF}~\citep{zhang2022arf} to controllable stylization for 3DGS. \emph{SGSST}~\citep{galerne2025sgsst} scales 3DGS stylization to ultra-high resolutions via multiscale losses. \emph{InstantStyleGaussian}~\citep{yu2024instantstylegaussian} accelerates the process by generating target-style images via diffusion and integrating them into the training set to iteratively optimize the 3DGS scene. However, most works require dense posed inputs and lengthy per-scene optimization, which fundamentally limits scalability and generalization to unseen environments. To this end, a concurrent work \emph{Styl3R} \cite{wang2025styl3rinstant3dstylized} proposes a pipeline that disentangles structure and appearance, unifying 3D reconstruction and style transfer in a single network. In contrast to Styl3R, which is restricted to 2-8 content views, our work generalizes from a single to arbitrary many context inputs, and further introduces a voxel-based 3D style loss to enforce cross-view coherence. Our dual-stream design explicitly disentangles geometry and style, enabling zero-shot stylization of unseen scenes.  





%Early progress framed 3D stylization as style injection into a NeRF scene via a \emph{hypernetwork}, which maps a reference style image to scene-conditioned parameters and is trained with a two-stage schedule and patch subsampling for efficiency~\citep{chiang2022stylizing}. This design enables coherent stylized novel views, but it still relies on per-scene optimization and known camera poses. \emph{StyleRF} then performs style transformation in the radiance-field feature space, improving geometry and supporting zero-shot transfer to new styles, though it remains radiance-field–based and computationally heavy~\citep{liu2023stylerf}. \emph{StyleGaussian} leverages 3D Gaussian Splatting to reach real-time rendering with multi-view consistency, and \emph{SGSST} scales 3DGS stylization to ultra-high resolutions via multiscale losses~\citep{liu2024stylegaussian, galerne2025sgsst}. Despite these advances, all of the above are \emph{scene-specific}: they require training or optimization on each individual scene, which fundamentally limits scalability and generalization to unseen environments.

%A concurrent work, Styl3R~\citep{wang2025styl3rinstant3dstylized}, adopts a dual-branch architecture that separates structure and appearance. Its structure branch leverages DUSt3R~\citep{wang2024dust3r} priors with a ViT encoder–decoder and cross-view attention to regress Gaussian geometry, while its appearance branch employs an independent style encoder and a stylization decoder where style tokens cross-attend to globally-aggregated content tokens. Although capable of zero-shot stylization, this design increases model complexity due to separate encoders, and its reliance on global-only attention for multi-view content aggregation may limit the recovery of fine-grained frame-level details.





















==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/sections/related_work_short.tex <==
\section{Related Work}

\subsection{Pose-free 3D Reconstruction}
%The feasibility of learning-based 3D reconstruction has been demonstrated in early CNN models~\citep{ummenhofer2017demon, zhou2018deeptam, teed2020deepv2d}.
3D reconstruction from unposed multi-view images or videos has drawn significant attention with the development of feed-forward models, including NeRF-based methods~\citep{smith2023flowcam,hong2024unifying} and 3DGS-based approaches~\citep{li2024ggrt,kim2025pf3plat}. 
DUSt3R~\citep{wang2024dust3r}, a Transformer-based framework, advances this direction by enabling pointmap estimation directly from image pairs. 
Its extensions~\citep{wang2024spann3r,yang2025fast3r,wang2025continuous,cabon2025must3r} further reduce reliance on global alignment procedures and support a varying number of input views. 
VGGT~\citep{wang2025vggt}, a recent 3D foundation model, revolutionizes this line of work by jointly predicting camera parameters, depth, point maps, and tracks from one to hundreds of views in a single forward pass, without any pose optimization.
\
As a follow-up to VGGT, AnySplat~\citep{jiang2025anysplat} introduces a rendering head and complements this design with a novel feed-forward Gaussian splatting pipeline, enabling the prediction of Gaussian primitives along with depth and camera parameters from uncalibrated images.

% \subsection{3D Style Transfer and losses}
% Explicit-representation approaches to 3D stylization~\citep{kato2018neural,cao2020psnet,guo2021volumetric,huang2021learning,hollein2022stylemesh,mu20223d} have shown promising results, 
% but their reliance on accurate geometry limits their applicability in complex real-world scenes.

% Implicit neural representations like NeRF~\citep{mildenhall2020nerf} have made 3D scene stylization more geometry-consistent,
% inspiring a range of methods that adapt NeRF through stylized view supervision or auxiliary networks~\citep{Nguyen2022SNeRF, zhang2022arf, chiang2022stylizing, huang2022stylizednerf}.
% StyleRF~\citep{liu2023stylerf} improves geometric fidelity and enables zero-shot transfer to unseen styles by applying style transformation in the radiance-field feature space.

% Recently, 3D Gaussian Splatting (3DGS)~\citep{kerbl20233d} has emerged as an efficient alternative to NeRF.
% Among stylization efforts, 
% StyleGaussian~\citep{liu2024stylegaussian} extends 3DGS with efficient feature rendering to enable real-time and view-consistent stylization,
% while subsequent works refine 3DGS for specialized stylization settings and efficiency improvements~\citep{mei2024regs,zhang2025stylizedgs,yu2024instantstylegaussian, galerne2025sgsst}.

% Concurrently, Styl3R~\citep{wang2025styl3r} builds on DUSt3R with two separate encoders that explicitly disentangle geometry and style at the feature extraction stage, but is restricted to 2–8 input views. 
% In contrast, Stylos follows the shared-backbone paradigm of AdaIN~\citep{huang2017arbitrary}, leveraging VGGT for unified feature extraction with head-level disentanglement of geometry and style,
% and supports content inputs ranging from a single view to hundreds of views.

% \subsection{Style Transfer Losses}

% Classical style transfer formulates style with Gram-matrix correlations~\citep{gatys2017image}.
% \cite{li2018demystifying} shows that 
% channel-wise mean and variance capture style information, leading to statistics-based style objectives.
% Similar to this insight, AdaIN~\citep{huang2018arbitrary} aligns content features to the statistics of a style reference, 
% achieving efficient arbitrary transfer.
% Extensions to video and multi-view stylization~\citep{ruder2017artistic, gupta2017characterizing, Nguyen2022SNeRF, zhang2022arf} 
% address temporal and cross-view consistency, while CLIP-based losses~\citep{radford2022learning} 
% encourage semantic alignment with text or image prompts. 

% Yet most of these objectives remain inherently 3D, computed per image or across concatenated views, 
% and thus cannot ensure consistency in complex real-world 4D scenes. 
% We instead extend statistics-based style losses into voxel space, introducing a 4D-aware objective that aligns feature distributions after multi-view fusion. 
% This formulation complements perceptual and CLIP-based losses, enforcing geometry-aware and view-consistent stylization.

\subsection{3D Style Transfer and Losses}
%Explicit-representation approaches to 3D stylization~\citep{kato2018neural,cao2020psnet,guo2021volumetric,huang2021learning,hollein2022stylemesh,mu20223d} have shown promising results, but their reliance on accurate geometry limits applicability in complex real-world scenes. Implicit neural representations like NeRF~\citep{mildenhall2020nerf} improve geometric consistency, inspiring a range of stylization methods based on stylized view supervision or auxiliary networks~\citep{Nguyen2022SNeRF, zhang2022arf, chiang2022stylizing, huang2022stylizednerf}. StylizedNeRF~\citep{huang2022stylizednerf} addresses the domain gap between style images and NeRF by introducing a mutual learning framework. StyleRF~\citep{liu2023stylerf} further enables zero-shot transfer by applying style transformations in radiance-field feature space. However, training NeRF for scene reconstruction is typically computationally expensive, making NeRF-based 3D stylization far from real-time.
3D stylization methods can be classified based on geometric representations, such as mesh~\citep{kato2018neural,liu2018paparazzi}, volumetric data~\citep{kim2019transport,kim2020lagrangian,guo2021volumetric}, point coulds~\citep{cao2020psnet,huang2021learning}. In addition, neural radiance fields (NeRF)~\citep{mildenhall2020nerf}, using an MLP to implicitly learn a static 3D scene, has inspired a range of stylization methods based on stylized view supervision or auxiliary networks~\citep{Nguyen2022SNeRF, zhang2022arf, chiang2022stylizing, huang2022stylizednerf}. StylizedNeRF~\citep{huang2022stylizednerf} addresses the domain gap between style images and NeRF by introducing a mutual learning framework. StyleRF~\citep{liu2023stylerf} further enables zero-shot transfer by applying style transformations in radiance-field feature space. However, training NeRFs for scene reconstruction and stylization is relatively computationally expensive, making NeRF-based 3D stylization far from real-time.

More recently, 3D Gaussian Splatting (3DGS)~\citep{kerbl20233d} has emerged as an efficient alternative to NeRF for 3D scene modeling.
Subsequent works refine 3DGS for efficient stylization~\citep{mei2024regs,kovacs2024gstyle,yu2024instantstylegaussian,zhang2025stylizedgs,galerne2025sgsst,lin2025multi}.
StyleGaussian~\citep{liu2024stylegaussian} extends 3DGS with efficient feature rendering to enable real-time zero-shot stylization. However, despite being significantly faster to optimize than NeRF, 3DGS-based approaches still require per-scene fitting, which poses a fundamental barrier to achieving truly real-time 3D stylization.
\
Styl3R~\citep{wang2025styl3r}, the closest contemporaneous related work to ours, introduces a feedforward framework for instant 3D stylized reconstruction. While effective and efficient, Styl3R is primarily designed for 2–8 input views and does not specifically target strong multi-view consistency among the rendered stylization results.

Underlying these architectures, style transfer objectives play a crucial role. 
Classical style transfer relies on Gram-matrix correlations~\citep{gatys2016image}, while channel-wise statistics such as mean and variance~\citep{li2017demystifying} offer efficient alternatives, forming the basis of AdaIN~\citep{huang2017arbitrary}. 
Extensions to video and multi-view stylization~\citep{ruder2016artistic, gupta2017characterizing, Nguyen2022SNeRF, zhang2022arf} address temporal and cross-view consistency, and CLIP-based losses~\citep{radford2021learning} introduce semantic alignment with text or image prompts. 
However, most objectives remain inherently 2D and cannot guarantee consistency across complex 3D scenes. 
To this end, we extend statistics-based style losses into voxel space, introducing a 3D-aware objective that aligns feature distributions after multi-view fusion. 
%This formulation complements perceptual and CLIP-based losses, enforcing geometry-aware and view-consistent stylization.


==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/sections/reproducibility_statement.tex <==
%\newpage
\section{Reproducibility Statement}

We have taken several steps to ensure the reproducibility of our work. 
The main paper describes all model architectures in Sec.~\ref{sec:method}. 
We provide detailed pseudo-code for the proposed 3D style loss function in Algo.~\ref{alg:3d_loss}, and will release the full implementation upon acceptance.
All datasets used are publicly available, as described in Sec.~\ref{sec:exp}. 
These resources should allow researchers to reproduce and extend our findings. 
In Appendix~\ref{appendix:rep_exp}, we clarify the training and inference details of the state-of-the-art methods for reproducible comparisons.
In addition, we provide extensive qualitative results in Appendix~\ref{appendix:visual}, 
and analyze efficiency trends with respect to the number of views per batch in Appendix~\ref{appendix:efficiency}, where efficiency experiments are averaged over 100 iterations per setting.

==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/tables/abl_frame_global.tex <==
\begin{table}[tb]
  \setlength{\tabcolsep}{0.12cm}
    \centering 
    \caption{Ablation on the style-content fusion module, comparing Frame, Global and hybrid CrossBlock designs.
    The first frame of each content scene is used as the pseudo style reference. Reconstruction quality is evaluated with PSNR$\uparrow$, SSIM$\uparrow$, and LPIPS$\downarrow$ on the CO3D dataset.}
    
  \begin{tabular}{c c c c c c c c c c c}
    \toprule
    \multicolumn{2}{c}{Strategies} 
      & \multicolumn{3}{c}{Skateboard} 
      & \multicolumn{3}{c}{Pizza} 
      & \multicolumn{3}{c}{Donut} \\
    \cmidrule(lr){1-2} \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
    Global & Frame 
      & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ 
      & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$
      & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ \\
    \midrule
    \checkmark & \checkmark 
      & {21.12} & {0.6858} & {0.2821} 
      & {19.78} & {0.5939} & {0.3326} 
      & {21.39} & {0.7198} & {0.3264} \\
     & \checkmark 
      & 20.93 & 0.6917 & 0.2912 
      & 19.72 & 0.5940 & 0.3405 
      & 21.40 & 0.7167 & 0.3340 \\
    \rowcolor{lightgray} \checkmark &  
      & \bftab21.68 & \bftab0.7043 & \bftab0.2684 
      & \bftab20.57 & \bftab0.6177 & \bftab0.3110 
      & \bftab22.09 & \bftab0.7362 & \bftab0.3125 \\
    \bottomrule
  \end{tabular}
  \label{tab:frame_global}
\end{table}

==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/tables/abl_losses.tex <==
\begin{table}[tb]
  \centering
  \caption{Consistency and artistic comparison of style loss designs on the CO3D test scenes.}
  \begin{tabular}{l c c c c | c}
    \toprule
    \multirow{2}{*}{Style Loss} & \multicolumn{2}{c}{Short-range} & \multicolumn{2}{c|}{Long-range} & \multirow{2}{*}{ArtScore$\uparrow$} \\
    \cmidrule(l){2-3} \cmidrule(l){4-5}
     & LPIPS$\downarrow$ & RMSE$\downarrow$ & LPIPS$\downarrow$ & RMSE$\downarrow$ & \\
    \midrule
    Image loss (Eq.~\ref{eq:img_loss})& 0.046 & 0.035 & 0.147 & 0.135 & 5.96\\
    Scene loss (Eq.~\ref{eq:scn_loss})& 0.048 & 0.037 & 0.147 & 0.133 & 9.54\\
    \rowcolor{lightgray} \bftab 3D loss (Eq.~\ref{eq:3d_loss}) & \bftab 0.046 & \bftab 0.033 & \bftab 0.140 & \bftab 0.128 & \bftab 9.62\\
    \bottomrule
  \end{tabular}
  \label{tab:style_loss}
\end{table}


==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/tables/abl_losses_final.tex <==
\begin{table}[tb]
  \centering
  \caption{Comparison of consistency and artistic quality among different style loss designs on CO3D. The frame stride is set to 3, and 15 held-out scenes are randomly selected for evaluation.}
  \begin{tabular}{l c c c c | c}
    \toprule
    \multirow{2}{*}{Style Loss} & \multicolumn{2}{c}{Short-range} & \multicolumn{2}{c|}{Long-range} & \multirow{2}{*}{ArtScore$\uparrow$} \\
    \cmidrule(l){2-3} \cmidrule(l){4-5}
     & LPIPS$\downarrow$ & RMSE$\downarrow$ & LPIPS$\downarrow$ & RMSE$\downarrow$ & \\
    \midrule
    Image loss (Eq.~\ref{eq:img_loss})& 0.048 & 0.038 & 0.157 & \bftab 0.142 & 4.78\\
    Scene loss (Eq.~\ref{eq:scn_loss})& \bftab 0.047 & 0.036 & 0.156 & 0.148 & 9.12\\
    \rowcolor{lightgray} \bftab 3D loss (Eq.~\ref{eq:3d_loss}) & \bftab 0.047 & \bftab 0.034 & \bftab 0.153 & \bftab 0.142 & \bftab 9.15\\
    \bottomrule
  \end{tabular}
  \label{tab:style_loss}
\end{table}


==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/tables/abl_losses_old.tex <==
\begin{table}[th]
  \centering
  \caption{Consistency comparison of different style loss designs on CO3D. The 3D loss achieves the strongest short-range and long-range consistency.}
  \begin{tabular}{l c c c c c}
    \toprule
    \multirow{2}{*}{\bftab Style Loss} & \multicolumn{2}{c}{\bftab Short-range} & \multicolumn{2}{c}{\bftab Long-range} & \multirow{2}{*}{ArtScore$\uparrow$} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
     & LPIPS$\downarrow$ & RMSE$\downarrow$ & LPIPS$\downarrow$ & RMSE$\downarrow$ \\
    \midrule
    Image loss (Eq.~\ref{eq:img_loss})& 0.046 & 0.035 & 0.147 & 0.135 & 5.96\\
    Scene loss (Eq.~\ref{eq:scn_loss})& 0.048 & 0.037 & 0.147 & 0.133 & 9.54\\
    \rowcolor{lightgray} \bftab 3D loss (Eq.~\ref{eq:3d_loss}) & \bftab 0.046 & \bftab 0.033 & \bftab 0.140 & \bftab 0.128 & \bftab 9.62\\
    \bottomrule
  \end{tabular}
  \label{tab:style_loss}
\end{table}

==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/tables/artscore_artfid_time.tex <==
\begin{table}[tb]
  \centering
  \setlength{\tabcolsep}{0.15cm}
    \caption{
    Stylization quality, as measured by ArtScore and ArtFID (abbreviated as Score and FID respectively), and stylization time comparisons with recent 3D stylization models. \textbf{\textit{Stylos}} achieves consistently favorable metric scores across the four scenes. Additionally, we follow StyleID~\citep{chung2024style} and calculate additional metrics as reported in~\ref{appendix:stylization_quality} Table~\ref{tab:metrics_train_truck} and Table~\ref{tab:metrics_m60_garden}.
    }
  \begin{threeparttable}
  \begin{tabular}{l cc cc cc cc |c}
    \toprule
    \multirow{2}{*}{Method} 
      & \multicolumn{2}{c}{Train} 
      & \multicolumn{2}{c}{Truck}
      & \multicolumn{2}{c}{M60}
      & \multicolumn{2}{c|}{Garden}
      & \multirow{2}{*}{Time$\downarrow$} \\
    \cmidrule(lr){2-3}
    \cmidrule(lr){4-5}
    \cmidrule(lr){6-7}
    \cmidrule(lr){8-9}
      & Score$\uparrow$ & FID$\downarrow$
      & Score$\uparrow$ & FID$\downarrow$
      & Score$\uparrow$ & FID$\downarrow$
      & Score$\uparrow$ & FID$\downarrow$
      &  \\
    \midrule
    \rowcolor[HTML]{E1F2FB}
    StyleGaussian~\citeyear{liu2024stylegaussian}
      & 0.78 & 52.79  & 5.76 & 44.93  & 8.63 & 47.48  & \textbf{9.38} & 41.14  & 165 m\tnote{*} \\
      \rowcolor[HTML]{F1F9F9}
    G-Style~\citeyear{kovacs2024gstyle}
      & \textbf{9.52} & \textbf{23.24}  & \ul{9.67} & \textbf{22.15}  & \textbf{9.73} & \textbf{22.36}  & 8.98 & \textbf{25.76}  & 14.7 m\tnote{*} \\
    \rowcolor[HTML]{F1F9F9}
    %StylizedGS~\citeyear{zhang2024stylizedgs}
    % & 4.95 & 40.79  & 6.45 & 42.07  & 7.39 & 53.24  & 6.99 & 65.15  & 13.3 m\tnote{*} \\
    %& 4.95 & -  & 6.45 & -  & 7.39 & -  & 6.99 & -  & 13.3 m\tnote{*} \\
    \rowcolor[HTML]{F1F9F9}SGSST~\citeyear{galerne2025sgsst}
      & 1.84 & 38.24  & 5.34 & 32.34  & 5.26 & 38.73  & 4.89 & 33.54  & 35.2 m\tnote{*} \\
    %Styl3R~\citeyear{wang2025styl3r}
    %  & 0.28 & --  & 2.94 & --  & 2.96 & --  & 4.09 & --  & 0.16 s\tnote{\textdagger} \\
   \rowcolor[HTML]{F5EFFF}Styl3R~\citeyear{wang2025styl3r}
      & -- & --  & 2.94 & 34.11  & 2.96 & 29.86  & 4.09 & 38.28  & \ul{0.16} s\tnote{\textdagger} \\
    \midrule
    \rowcolor[HTML]{F5EFFF}
    \textbf{\textit{Stylos}} (ours)
      & \ul{9.50} & \ul{26.40} 
      & \textbf{9.70} & \ul{28.71} 
      & \ul{9.37} & \ul{27.44} 
      & \ul{9.34} & \ul{28.06} 
      & \textbf{0.05} s\tnote{\textdagger} \\
    \bottomrule
  \end{tabular}
  \begin{tablenotes}
  \footnotesize
  \item[*] For methods with per-scene fitting required, the training phase accounts towards stylization time (see~\ref{appendix:stylization_time}).
  \item[\textdagger] As to single-forward 3D stylization approaches, training is not considered for stylization time.
  %The proposed Stylos exhibits competitive stylization quality with improved efficiency.
  %\item[\textdagger] Styl3R (with default pose optimization) runs at 0.88 s per image at an input resolution of $256\times256$.
  %\item[\textsection] Stylos remains $3\times$ faster than Styl3R (w/o default pose optimization) at an input size of $448\times448$.
  \end{tablenotes}
  \end{threeparttable}
  \label{tab:artscore}
\end{table}


==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/tables/artscore_old.tex <==
\begin{table}[tb]
  \centering
  \setlength{\tabcolsep}{0.15cm}
  \caption{ArtScore$\uparrow$ comparison across methods on four Tanks and Temples scenes.}
  \begin{tabular}{l c c c c}
    \toprule
    \bftab Method & \bftab Train & \bftab Truck & \bftab M60 & \bftab Garden \\
    \midrule
    StyleRF~\citeyear{liu2023stylerf} & 7.71 & 4.12 & 8.48 & -- \\
    StyleGS~\citeyear{liu2024stylegaussian} & 0.78 & 5.76 & 8.63 & \bftab 9.38 \\
    \rowcolor{lightgray} Stylos (ours) & \bftab 9.50 & \bftab 9.70 & \bftab 9.37 & 9.34 \\
    \bottomrule
  \end{tabular}
  \label{tab:artscore}
\end{table}

==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/tables/artscore_time.tex <==
\begin{table}[tb]
  \centering
  \setlength{\tabcolsep}{0.12cm}
    \caption{
    Stylization scores and time comparisons with recent 3D stylization models on four Tanks \& Temples scenes. Refer to~\ref{appendix:stylization_time} for study details.
    }
  \begin{tabular}{l c c c c c}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{4}{c}{ArtScore$\uparrow$} 
    & Stylization Time \\
    \cmidrule(lr){2-5}
     &
    Train &
    Truck &
    M60 &
    Garden &
    seconds/image \\
    \midrule
    %StylizedNeRF~\citeyear{huang2022stylizednerf}
    %  & -9.32 & -10.36 & -9.80 & -9.38 
    %  & 17.0 & 17.5 \\
    GStyle~\citeyear{kovacs2024gstyle}
      & 9.70 & 9.76 & 9.89 & 9.18 & -- \\
    StyleGaussian~\citeyear{liu2024stylegaussian}
      & 0.78 & 5.76 & 8.63 & 9.38 & -- \\
    StylizedGS$^*$~\citeyear{zhang2024stylizedgs}
      & 4.95 & 6.45 & 7.39 & 6.99 & -- \\
    SGSST~\citeyear{galerne2025sgsst}
      & 1.84 & 5.34 & 5.26 & 4.89 & -- \\
    Styl3R~\citeyear{wang2025styl3rinstant3dstylized}
      & 0.28 & 2.94 & 2.96 & 4.09 & -- \\
    \rowcolor{lightgray}
    \textbf{\textit{Stylos}} (ours)
      & 9.50 & 9.70 & 9.37 & 9.34 & 0.046 \\
    \bottomrule
  \end{tabular}
  \label{tab:artscore}
\end{table}


==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/tables/consistency.tex <==
\begin{table}[tb]
  \centering
  \setlength{\tabcolsep}{0.12cm}
  \caption{For consistency comparisons, we report short-range and long-range LPIPS$\downarrow$ and RMSE$\downarrow$ on the four scenes from the Tanks \& Temples dataset. We clarify experiment details in~\ref{appendix:stylization_quality}. In the following tables, the best results are {\bftab highlighted} and the second best results are \ul{underlined}. Each stylization method category is visualized with a distinct color. The proposed \textbf{\textit{Stylos}} demonstrates improved short-range and long-range consistency scores across the four scenes.}
  \begin{threeparttable}
  \begin{tabular}{l c c c c c c c c}
    \toprule
    \multirow{2}{*}{Method} &
      \multicolumn{2}{c}{Train} &
      \multicolumn{2}{c}{Truck} &
      \multicolumn{2}{c}{M60} &
      \multicolumn{2}{c}{Garden} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
     & LPIPS$\downarrow$ & RMSE$\downarrow$
     & LPIPS$\downarrow$ & RMSE$\downarrow$
     & LPIPS$\downarrow$ & RMSE$\downarrow$
     & LPIPS$\downarrow$ & RMSE$\downarrow$ \\
    \midrule
    \multicolumn{9}{c}{\it Short-range consistency} \\
    \midrule
    %StylizedNeRF ~\citeyear{huang2022stylizednerf} 
    %& 0.071 & 0.056 & 0.037 & 0.029 & 0.043 & 0.034 & 0.111 & 0.103 \\
    \rowcolor[HTML]{E1F2FB}
    StyleGaussian ~\citeyear{liu2024stylegaussian} 
    & \ul{0.033} & \ul{0.038} & \ul{0.031} & \ul{0.034} & \ul{0.038} & 0.037 & 0.069 & \ul{0.061} \\
    \rowcolor[HTML]{F1F9F9}
    G-Style ~\citeyear{kovacs2024gstyle} 
    & 0.042 & 0.052 & 0.032 & 0.035 & \ul{0.038} & \ul{0.034} & \ul{0.066} & 0.070 \\
    \rowcolor[HTML]{F1F9F9}
    %StylizedGS\tnote{*} ~\citeyear{zhang2025stylizedgs} 
    %& \bftab0.016 & \bftab0.023 & \bftab0.013 & \bftab0.019 & \bftab0.017 & \bftab0.020 & \ul{0.056} & \bftab0.041 \\
    \rowcolor[HTML]{F1F9F9}
    SGSST ~\citeyear{galerne2025sgsst} 
    & 0.038 & 0.047 & 0.039 & 0.047 & 0.044 & 0.049 & 0.084 & 0.090 \\
    %Styl3R~\citeyear{wang2025styl3r}
    %& 0.067 & 0.042 & 0.061 & 0.036 & 0.066 & 0.040 & 0.105 & 0.067 \\
    \rowcolor[HTML]{F5EFFF}
    Styl3R~\citeyear{wang2025styl3r}
    & -- & -- & 0.061 & 0.036 & 0.066 & 0.040 & 0.105 & 0.067 \\
    \midrule
    \rowcolor[HTML]{F5EFFF}
    \textbf{\textit{Stylos}} (ours) 
    & \textbf{0.030} & \textbf{0.026} & \textbf{0.028} & \textbf{0.021} & \textbf{0.035} & \textbf{0.024} & \textbf{0.047} & \textbf{0.044} \\
    %\rowcolor{lightgray}
    %\textbf{\textit{Stylos}} (ours new) 
    %& -- & -- & -- & -- & -- & -- & -- & -- \\
    \midrule
    \multicolumn{9}{c}{\it Long-range consistency} \\
    \midrule
    %StylizedNeRF ~\citeyear{huang2022stylizednerf} 
    %& 0.086 & 0.066 & 0.071 & 0.080 & 0.068 & \bftab0.054 & \ul{0.109} & \bftab0.100 \\
    \rowcolor[HTML]{E1F2FB}
    StyleGaussian ~\citeyear{liu2024stylegaussian} 
    & \ul{0.067} & \ul{0.072} & \ul{0.086} & \ul{0.077} & \ul{0.091} & \ul{0.091} & 0.177 & \ul{0.141} \\
    \rowcolor[HTML]{F1F9F9}
    G-Style ~\citeyear{kovacs2024gstyle} 
    & 0.098 & 0.120 & 0.095 & 0.093 & 0.104 & 0.095 & 0.180 & 0.175 \\
    \rowcolor[HTML]{F1F9F9}
    %StylizedGS\tnote{*} ~\citeyear{zhang2025stylizedgs} 
    %& \bftab0.040 & \ul{0.065} & \bftab0.049 & \bftab0.064 & \bftab0.065 & \ul{0.086} & \bftab0.100 & 0.202 \\
    \rowcolor[HTML]{F1F9F9}
    SGSST ~\citeyear{galerne2025sgsst} 
    & 0.087 & 0.108 & 0.119 & 0.120 & 0.130 & 0.128 & 0.221 & 0.222 \\
    %Styl3R ~\citeyear{wang2025styl3r} 
    %& 0.107 & 0.108 & 0.116 & 0.100 & 0.147 & 0.143 & 0.146 & 0.145 \\
    \rowcolor[HTML]{F5EFFF}
    Styl3R ~\citeyear{wang2025styl3r} 
    & -- & -- & 0.116 & 0.100 & 0.147 & 0.143 & \ul{0.146} & 0.145 \\
    % \rowcolor{lightgray}
    \midrule
    \rowcolor[HTML]{F5EFFF}
    \textbf{\textit{Stylos}} (ours) 
    & \textbf{0.051} & \textbf{0.056} & \textbf{0.074} & \textbf{0.069} & \textbf{0.083} & \textbf{0.082} & \textbf{0.139} & \textbf{0.134} \\
    %\rowcolor{lightgray}
    %\textbf{\textit{Stylos}} (ours new) 
    %& -- & -- & -- & -- & -- & -- & -- & -- \\
    \bottomrule
  \end{tabular}
  \begin{tablenotes}
  \footnotesize
  \item[] 
  % not sure the root cause of failure cases, better get rid of \textit{severe color smearing}
  StylizedGS~\citep{zhang2025stylizedgs} is not included in quantitative comparisons due to its multiple failure cases observed on our test styles. Nevertheless, its quantitative results are reported in~\ref{appendix:stylization_quality} Table~\ref{tab:metrics_train_truck} and Table~\ref{tab:metrics_m60_garden} for readers' reference. Reproduced results are available at https://github.com/HanzhouLiu/Stylos.
  \end{tablenotes}
  \end{threeparttable}
  \label{tab:consistency}
\end{table}


==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/tables/consistency_old.tex <==
\begin{table}[tb]
  \centering
  \setlength{\tabcolsep}{0.13cm}
  \caption{Consistency comparison across methods. 
  We report short-range (top) and long-range (bottom) LPIPS$\downarrow$ and RMSE$\downarrow$, on the four scenes from Tanks and Temples.}
  \begin{tabular}{l c c c c c c c c}
    \toprule
    \multirow{2}{*}{\bftab Method} & \multicolumn{2}{c}{\bftab Train} & \multicolumn{2}{c}{\bftab Truck} & \multicolumn{2}{c}{\bftab M60} & \multicolumn{2}{c}{\bftab Garden} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
     & LPIPS$\downarrow$ & RMSE$\downarrow$ & LPIPS$\downarrow$ & RMSE$\downarrow$ & LPIPS$\downarrow$ & RMSE$\downarrow$ & LPIPS$\downarrow$ & RMSE$\downarrow$ \\
    \midrule
    \multicolumn{9}{c}{\it Short-range consistency} \\
    \midrule
    StyleRF~\citeyear{liu2023stylerf} & 0.075 & 0.065 & 0.060 & 0.062 & 0.039 & 0.042 & -- & -- \\
    StyleGS~\citeyear{liu2024stylegaussian} & 0.033 & 0.038 & 0.031 & 0.034 & 0.038 & 0.037 & 0.069 & 0.061 \\
    \rowcolor{lightgray} Stylos (ours) & \bftab 0.030 & \bftab 0.026 & \bftab 0.028 & \bftab 0.021 & \bftab 0.035 & \bftab 0.024 & \bftab 0.047 & \bftab 0.044 \\
    \midrule
    \multicolumn{9}{c}{\it Long-range consistency} \\
    \midrule
    StyleRF~\citeyear{liu2023stylerf} & 0.116 & 0.110 & 0.176 & 0.154 & 0.096 & 0.092 & -- & -- \\
    StyleGS~\citeyear{liu2024stylegaussian} & 0.067 & 0.072 & 0.086 & 0.077 & 0.091 & 0.091 & 0.177 & 0.141 \\
    \rowcolor{lightgray} Stylos (ours) & \bftab 0.051 & \bftab 0.056 & \bftab 0.074 & \bftab 0.069 & \bftab 0.083 & \bftab 0.082 & \bftab 0.139 & \bftab 0.134 \\
    \bottomrule
  \end{tabular}
  \label{tab:consistency}
\end{table}

==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/iclr2026/tables/consistency_rebuttal.tex <==
\begin{table}[tb]
  \centering
  \setlength{\tabcolsep}{0.12cm}
  \caption{For consistency comparisons, we report short-range and long-range LPIPS$\downarrow$ and RMSE$\downarrow$ on the four scenes from the Tanks \& Temples dataset. We clarify experiment details in~\ref{appendix:stylization_quality}. In the following tables, the best results are {\bftab highlighted} and the second best results are \ul{underlined}. Each stylization method category is visualized with a distinct color.}
  \begin{threeparttable}
  \begin{tabular}{l c c c c c c c c}
    \toprule
    \multirow{2}{*}{Method} &
      \multicolumn{2}{c}{Train} &
      \multicolumn{2}{c}{Truck} &
      \multicolumn{2}{c}{M60} &
      \multicolumn{2}{c}{Garden} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
     & LPIPS$\downarrow$ & RMSE$\downarrow$
     & LPIPS$\downarrow$ & RMSE$\downarrow$
     & LPIPS$\downarrow$ & RMSE$\downarrow$
     & LPIPS$\downarrow$ & RMSE$\downarrow$ \\
    \midrule
    \multicolumn{9}{c}{\it Short-range consistency} \\
    \midrule
    %StylizedNeRF ~\citeyear{huang2022stylizednerf} 
    %& 0.071 & 0.056 & 0.037 & 0.029 & 0.043 & 0.034 & 0.111 & 0.103 \\
    \rowcolor[HTML]{E1F2FB}
    StyleGaussian ~\citeyear{liu2024stylegaussian} 
    & 0.033 & 0.038 & 0.031 & 0.034 & 0.038 & 0.037 & 0.069 & 0.061 \\
    \rowcolor[HTML]{F1F9F9}
    G-Style ~\citeyear{kovacs2024gstyle} 
    & 0.042 & 0.052 & 0.032 & 0.035 & 0.038 & 0.034 & 0.066 & 0.070 \\
    \rowcolor[HTML]{F1F9F9}
    StylizedGS\tnote{*} ~\citeyear{zhang2024stylizedgs} 
    & \bftab0.016 & \bftab0.023 & \bftab0.013 & \bftab0.019 & \bftab0.017 & \bftab0.020 & \ul{0.056} & \bftab0.041 \\
    \rowcolor[HTML]{F1F9F9}
    SGSST ~\citeyear{galerne2025sgsst} 
    & 0.038 & 0.047 & 0.039 & 0.047 & 0.044 & 0.049 & 0.084 & 0.090 \\
    %Styl3R~\citeyear{wang2025styl3rinstant3dstylized}
    %& 0.067 & 0.042 & 0.061 & 0.036 & 0.066 & 0.040 & 0.105 & 0.067 \\
    \rowcolor[HTML]{F5EFFF}
    Styl3R~\citeyear{wang2025styl3rinstant3dstylized}
    & -- & -- & 0.061 & 0.036 & 0.066 & 0.040 & 0.105 & 0.067 \\
    \midrule
    \rowcolor[HTML]{F5EFFF}
    \textbf{\textit{Stylos}} (ours) 
    & \ul{0.030} & \ul{0.026} & \ul{0.028} & \ul{0.021} & \ul{0.035} & \ul{0.024} & \bftab0.047 & \ul{0.044} \\
    %\rowcolor{lightgray}
    %\textbf{\textit{Stylos}} (ours new) 
    %& -- & -- & -- & -- & -- & -- & -- & -- \\
    \midrule
    \multicolumn{9}{c}{\it Long-range consistency} \\
    \midrule
    %StylizedNeRF ~\citeyear{huang2022stylizednerf} 
    %& 0.086 & 0.066 & 0.071 & 0.080 & 0.068 & \bftab0.054 & \ul{0.109} & \bftab0.100 \\
    \rowcolor[HTML]{E1F2FB}
    StyleGaussian ~\citeyear{liu2024stylegaussian} 
    & 0.067 & 0.072 & 0.086 & 0.077 & 0.091 & 0.091 & 0.177 & \ul{0.141} \\
    \rowcolor[HTML]{F1F9F9}
    G-Style ~\citeyear{kovacs2024gstyle} 
    & 0.098 & 0.120 & 0.095 & 0.093 & 0.104 & 0.095 & 0.180 & 0.175 \\
    \rowcolor[HTML]{F1F9F9}
    StylizedGS\tnote{*} ~\citeyear{zhang2024stylizedgs} 
    & \bftab0.040 & \ul{0.065} & \bftab0.049 & \bftab0.064 & \bftab0.065 & \ul{0.086} & \bftab0.100 & 0.202 \\
    \rowcolor[HTML]{F1F9F9}
    SGSST ~\citeyear{galerne2025sgsst} 
    & 0.087 & 0.108 & 0.119 & 0.120 & 0.130 & 0.128 & 0.221 & 0.222 \\
    %Styl3R ~\citeyear{wang2025styl3rinstant3dstylized} 
    %& 0.107 & 0.108 & 0.116 & 0.100 & 0.147 & 0.143 & 0.146 & 0.145 \\
    \rowcolor[HTML]{F5EFFF}
    Styl3R ~\citeyear{wang2025styl3rinstant3dstylized} 
    & -- & -- & 0.116 & 0.100 & 0.147 & 0.143 & 0.146 & 0.145 \\
    % \rowcolor{lightgray}
    \midrule
    \rowcolor[HTML]{F5EFFF}
    \textbf{\textit{Stylos}} (ours) 
    & \ul{0.051} & \bftab0.056 & \ul{0.074} & \ul{0.069} & \ul{0.083} & \textbf{0.082} & \ul{0.139} & \bftab0.134 \\
    %\rowcolor{lightgray}
    %\textbf{\textit{Stylos}} (ours new) 
    %& -- & -- & -- & -- & -- & -- & -- & -- \\
    \bottomrule
  \end{tabular}
  \begin{tablenotes}
  \footnotesize
  \item[*] For StylizedGS, cases with \textit{severe color smearing} are excluded when evaluating consistency and ArtScore. Refer to https://github.com/HanzhouLiu/Stylos for reproduced results and evaluation methods.
  \end{tablenotes}
  \end{threeparttable}
  \label{tab:consistency}
\end{table}


==> bsrbwtvmfdhvdqtkjrnpgpbtqzddtdbh/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr2026/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr2026/sections/limitation.tex <==
\section{Limitation}
The main limitations of Stylos are provided as follows. (1) We observe that using a large CLIP weight may overemphasize semantic alignment at the expense of fine-grained texture details. Developing more principled strategies for multi-loss balancing could further improve stylization fidelity. (2) Stylos can process entire scenes with dozens (even hundreds) of input views, but its computation cost and latency increase correspondingly, as analyzed in Appendix~\ref{appendix:efficiency}. 

==> iclr2026/sections/related_work.tex <==
\section{Related Work}


\subsection{Single-Forward 3D Reconstruction}
% Most NeRF and 3DGS methods assume access to accurate camera pose, which introduces an implicit preprocessing step that conceals the significant time and logistical costs of large-scale, multi-view data acquisition and registration. To overcome these limitations,

Recent advances in 3D reconstruction have shifted from optimization-heavy pipelines to single-forward models that directly predict structure and camera parameters from raw images. Early CNN-based attempts such as \emph{DeMoN} \cite{ummenhofer2017demon}, \emph{DeepTAM} \cite{zhou2018deeptam} and \emph{DeepV2D} \cite{Teed2020DeepV2D:} demonstrate feasibility but fell short of classical methods. The transformer era brought large-scale models like DUSt3R \cite{wang2024dust3r} and its extension MASt3R \cite{leroy2024grounding}, which replaced multi-stage SfM pipelines with single-pass predictions of geometry and poses. While effective, these models require expensive post-processing and often struggle with alignment in complex multi-view settings. Subsequent works such as Spann3R \cite{wang2024spann3r},CUT3R \cite{wang2025continuous} and MUSt3R \cite{cabon2025must3r} reduced reliance on classical optimization by incorporating memory or parallelized attention but incurred high computational costs at the same time. More recently, VGGT \cite{wang2025vggt} introduced alternating-attention transformers for joint multi-view inference of depth, pose and pointmaps, which achieves more consistent and scalable resonctructions. In parallel, feed-forward Gaussian splatting methods like AnySplat \cite{jiang2025anysplat} demonstrate that end-to-end pipelines can jointly recover geometry, camera intrinsics and novel views directly from uncalibrated images. Our work is inspired by such methods and aims to extend them to 3D style transfer. 


\subsection{3D Style Transfer}
% 3D scene stylizing has attracted growing research efforts.
Early works have achieved impressive 3D scene style transfer results over diverse explicit representations such as mesh~\citep{kato2018neural,michel2022text2mesh,Hollein_2022_CVPR}, voxel~\citep{guo2021volumetric} and point cloud~\citep{huang2021learning,mu20223d,cao2020psnet}. However, the quality of their results is limited by the precision of the geometric reconstructions, which often leads to noticeable artifacts in complex real-world scenes. 

The advent of implicit neural representations like Neural Radiance Fields (NeRF)~\citep{mildenhall2020nerf} has provided a more visually compelling and geometry-consistent results for 3D scene stylization. \cite{Nguyen2022SNeRF} use individually stylized
images rendered from a pre-trained NeRF as targets, iteratively fine-tuning the model to align with the desired style in a view-consistent manner. \emph{ARF} \cite{zhang2022arf} 
follows a similar approach but employs a nearest neighbor matching loss on the features extracted from rendering
and style instead of a standard color loss.
%transfers artistic features from 2D style images to 3D scenes, treating stylization as an optimization problem within the NeRF framework. 
To allow for zero-shot style transfer,~\citep{chiang2022stylizing}frames 3D stylization as style injection into a NeRF scene via a hypernetwork, which maps a reference style image to scene-conditioned parameters. \emph{StylizedNeRF}~\citep{huang2022stylizednerf} jointly learns 2D and 3D stylization. \emph{StyleRF}~\citep{liu2023stylerf} then performs style transformation in the radiance-field feature space, improving geometry and supporting zero-shot transfer to new styles. Despite these advances, NeRF-based methods remain computationally expensive, the rendering speed is limited by their volumetric nature, which restrict their usability in real-time scenarios. 
%requiring dense posed inputs and lengthy per-scene optimization, which restrict their usability in interactive or casual scenarios. 
%StyleRF learns high level features in 3D space for fast zero-shot style transfer.

Recently, 3D Gaussian Splatting (3DGS) \cite{kerbl20233d} has emerged as a promising explicit yet efficient representation for stylization. Unlike NeRFs, 3DGS enables real-time rendering while maintaining high reconstruction quality. \emph{ReGS} \cite{mei2024regs} refines a pre-trained 3DGS to a single style using a texture-guided control mechanism. \emph{StyleGaussian}~\citep{liu2024stylegaussian} proposes an efficient feature rendering strategy capable of swiftly rendering high-dimensional VGG features. 
% avoid per-asset optimization by embedding VGG features into each Gaussian splat which are then modulated based on a target style image and decoded back to stylized colors. 
\emph{StylizedGS}~\citep{zhang2024stylizedgs} is an optimization-based method that extends \emph{ARF}~\citep{zhang2022arf} to controllable stylization for 3DGS. \emph{SGSST}~\citep{galerne2025sgsst} scales 3DGS stylization to ultra-high resolutions via multiscale losses. \emph{InstantStyleGaussian}~\citep{yu2024instantstylegaussian} accelerates the process by generating target-style images via diffusion and integrating them into the training set to iteratively optimize the 3DGS scene. However, most works require dense posed inputs and lengthy per-scene optimization, which fundamentally limits scalability and generalization to unseen environments. To this end, a concurrent work \emph{Styl3R} \cite{wang2025styl3rinstant3dstylized} proposes a pipeline that disentangles structure and appearance, unifying 3D reconstruction and style transfer in a single network. In contrast to Styl3R, which is restricted to 2-8 content views, our work generalizes from a single to arbitrary many context inputs, and further introduces a voxel-based 3D style loss to enforce cross-view coherence. Our dual-stream design explicitly disentangles geometry and style, enabling zero-shot stylization of unseen scenes.  





%Early progress framed 3D stylization as style injection into a NeRF scene via a \emph{hypernetwork}, which maps a reference style image to scene-conditioned parameters and is trained with a two-stage schedule and patch subsampling for efficiency~\citep{chiang2022stylizing}. This design enables coherent stylized novel views, but it still relies on per-scene optimization and known camera poses. \emph{StyleRF} then performs style transformation in the radiance-field feature space, improving geometry and supporting zero-shot transfer to new styles, though it remains radiance-field–based and computationally heavy~\citep{liu2023stylerf}. \emph{StyleGaussian} leverages 3D Gaussian Splatting to reach real-time rendering with multi-view consistency, and \emph{SGSST} scales 3DGS stylization to ultra-high resolutions via multiscale losses~\citep{liu2024stylegaussian, galerne2025sgsst}. Despite these advances, all of the above are \emph{scene-specific}: they require training or optimization on each individual scene, which fundamentally limits scalability and generalization to unseen environments.

%A concurrent work, Styl3R~\citep{wang2025styl3rinstant3dstylized}, adopts a dual-branch architecture that separates structure and appearance. Its structure branch leverages DUSt3R~\citep{wang2024dust3r} priors with a ViT encoder–decoder and cross-view attention to regress Gaussian geometry, while its appearance branch employs an independent style encoder and a stylization decoder where style tokens cross-attend to globally-aggregated content tokens. Although capable of zero-shot stylization, this design increases model complexity due to separate encoders, and its reliance on global-only attention for multi-view content aggregation may limit the recovery of fine-grained frame-level details.





















==> iclr2026/tables/abl_losses.tex <==
\begin{table}[tb]
  \centering
  \caption{Consistency and artistic comparison of style loss designs on the CO3D test scenes.}
  \begin{tabular}{l c c c c | c}
    \toprule
    \multirow{2}{*}{Style Loss} & \multicolumn{2}{c}{Short-range} & \multicolumn{2}{c|}{Long-range} & \multirow{2}{*}{ArtScore$\uparrow$} \\
    \cmidrule(l){2-3} \cmidrule(l){4-5}
     & LPIPS$\downarrow$ & RMSE$\downarrow$ & LPIPS$\downarrow$ & RMSE$\downarrow$ & \\
    \midrule
    Image loss (Eq.~\ref{eq:img_loss})& 0.046 & 0.035 & 0.147 & 0.135 & 5.96\\
    Scene loss (Eq.~\ref{eq:scn_loss})& 0.048 & 0.037 & 0.147 & 0.133 & 9.54\\
    \rowcolor{lightgray} \bftab 3D loss (Eq.~\ref{eq:3d_loss}) & \bftab 0.046 & \bftab 0.033 & \bftab 0.140 & \bftab 0.128 & \bftab 9.62\\
    \bottomrule
  \end{tabular}
  \label{tab:style_loss}
\end{table}


==> iclr2026/tables/abl_losses_old.tex <==
\begin{table}[th]
  \centering
  \caption{Consistency comparison of different style loss designs on CO3D. The 3D loss achieves the strongest short-range and long-range consistency.}
  \begin{tabular}{l c c c c c}
    \toprule
    \multirow{2}{*}{\bftab Style Loss} & \multicolumn{2}{c}{\bftab Short-range} & \multicolumn{2}{c}{\bftab Long-range} & \multirow{2}{*}{ArtScore$\uparrow$} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5}
     & LPIPS$\downarrow$ & RMSE$\downarrow$ & LPIPS$\downarrow$ & RMSE$\downarrow$ \\
    \midrule
    Image loss (Eq.~\ref{eq:img_loss})& 0.046 & 0.035 & 0.147 & 0.135 & 5.96\\
    Scene loss (Eq.~\ref{eq:scn_loss})& 0.048 & 0.037 & 0.147 & 0.133 & 9.54\\
    \rowcolor{lightgray} \bftab 3D loss (Eq.~\ref{eq:3d_loss}) & \bftab 0.046 & \bftab 0.033 & \bftab 0.140 & \bftab 0.128 & \bftab 9.62\\
    \bottomrule
  \end{tabular}
  \label{tab:style_loss}
\end{table}

==> iclr2026/tables/artscore_old.tex <==
\begin{table}[tb]
  \centering
  \setlength{\tabcolsep}{0.15cm}
  \caption{ArtScore$\uparrow$ comparison across methods on four Tanks and Temples scenes.}
  \begin{tabular}{l c c c c}
    \toprule
    \bftab Method & \bftab Train & \bftab Truck & \bftab M60 & \bftab Garden \\
    \midrule
    StyleRF~\citeyear{liu2023stylerf} & 7.71 & 4.12 & 8.48 & -- \\
    StyleGS~\citeyear{liu2024stylegaussian} & 0.78 & 5.76 & 8.63 & \bftab 9.38 \\
    \rowcolor{lightgray} Stylos (ours) & \bftab 9.50 & \bftab 9.70 & \bftab 9.37 & 9.34 \\
    \bottomrule
  \end{tabular}
  \label{tab:artscore}
\end{table}

==> iclr2026/tables/artscore_time.tex <==
\begin{table}[tb]
  \centering
  \setlength{\tabcolsep}{0.12cm}
    \caption{
    Stylization scores and time comparisons with recent 3D stylization models on four Tanks \& Temples scenes. Refer to~\ref{appendix:stylization_time} for study details.
    }
  \begin{tabular}{l c c c c c}
    \toprule
    \multirow{2}{*}{Method} & \multicolumn{4}{c}{ArtScore$\uparrow$} 
    & Stylization Time \\
    \cmidrule(lr){2-5}
     &
    Train &
    Truck &
    M60 &
    Garden &
    seconds/image \\
    \midrule
    %StylizedNeRF~\citeyear{huang2022stylizednerf}
    %  & -9.32 & -10.36 & -9.80 & -9.38 
    %  & 17.0 & 17.5 \\
    GStyle~\citeyear{kovacs2024gstyle}
      & 9.70 & 9.76 & 9.89 & 9.18 & -- \\
    StyleGaussian~\citeyear{liu2024stylegaussian}
      & 0.78 & 5.76 & 8.63 & 9.38 & -- \\
    StylizedGS$^*$~\citeyear{zhang2024stylizedgs}
      & 4.95 & 6.45 & 7.39 & 6.99 & -- \\
    SGSST~\citeyear{galerne2025sgsst}
      & 1.84 & 5.34 & 5.26 & 4.89 & -- \\
    Styl3R~\citeyear{wang2025styl3rinstant3dstylized}
      & 0.28 & 2.94 & 2.96 & 4.09 & -- \\
    \rowcolor{lightgray}
    \textbf{\textit{Stylos}} (ours)
      & 9.50 & 9.70 & 9.37 & 9.34 & 0.046 \\
    \bottomrule
  \end{tabular}
  \label{tab:artscore}
\end{table}


==> iclr2026/tables/consistency_old.tex <==
\begin{table}[tb]
  \centering
  \setlength{\tabcolsep}{0.13cm}
  \caption{Consistency comparison across methods. 
  We report short-range (top) and long-range (bottom) LPIPS$\downarrow$ and RMSE$\downarrow$, on the four scenes from Tanks and Temples.}
  \begin{tabular}{l c c c c c c c c}
    \toprule
    \multirow{2}{*}{\bftab Method} & \multicolumn{2}{c}{\bftab Train} & \multicolumn{2}{c}{\bftab Truck} & \multicolumn{2}{c}{\bftab M60} & \multicolumn{2}{c}{\bftab Garden} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
     & LPIPS$\downarrow$ & RMSE$\downarrow$ & LPIPS$\downarrow$ & RMSE$\downarrow$ & LPIPS$\downarrow$ & RMSE$\downarrow$ & LPIPS$\downarrow$ & RMSE$\downarrow$ \\
    \midrule
    \multicolumn{9}{c}{\it Short-range consistency} \\
    \midrule
    StyleRF~\citeyear{liu2023stylerf} & 0.075 & 0.065 & 0.060 & 0.062 & 0.039 & 0.042 & -- & -- \\
    StyleGS~\citeyear{liu2024stylegaussian} & 0.033 & 0.038 & 0.031 & 0.034 & 0.038 & 0.037 & 0.069 & 0.061 \\
    \rowcolor{lightgray} Stylos (ours) & \bftab 0.030 & \bftab 0.026 & \bftab 0.028 & \bftab 0.021 & \bftab 0.035 & \bftab 0.024 & \bftab 0.047 & \bftab 0.044 \\
    \midrule
    \multicolumn{9}{c}{\it Long-range consistency} \\
    \midrule
    StyleRF~\citeyear{liu2023stylerf} & 0.116 & 0.110 & 0.176 & 0.154 & 0.096 & 0.092 & -- & -- \\
    StyleGS~\citeyear{liu2024stylegaussian} & 0.067 & 0.072 & 0.086 & 0.077 & 0.091 & 0.091 & 0.177 & 0.141 \\
    \rowcolor{lightgray} Stylos (ours) & \bftab 0.051 & \bftab 0.056 & \bftab 0.074 & \bftab 0.069 & \bftab 0.083 & \bftab 0.082 & \bftab 0.139 & \bftab 0.134 \\
    \bottomrule
  \end{tabular}
  \label{tab:consistency}
\end{table}

==> iclr2026/tables/consistency_rebuttal.tex <==
\begin{table}[tb]
  \centering
  \setlength{\tabcolsep}{0.12cm}
  \caption{For consistency comparisons, we report short-range and long-range LPIPS$\downarrow$ and RMSE$\downarrow$ on the four scenes from the Tanks \& Temples dataset. We clarify experiment details in~\ref{appendix:stylization_quality}. In the following tables, the best results are {\bftab highlighted} and the second best results are \ul{underlined}. Each stylization method category is visualized with a distinct color.}
  \begin{threeparttable}
  \begin{tabular}{l c c c c c c c c}
    \toprule
    \multirow{2}{*}{Method} &
      \multicolumn{2}{c}{Train} &
      \multicolumn{2}{c}{Truck} &
      \multicolumn{2}{c}{M60} &
      \multicolumn{2}{c}{Garden} \\
    \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
     & LPIPS$\downarrow$ & RMSE$\downarrow$
     & LPIPS$\downarrow$ & RMSE$\downarrow$
     & LPIPS$\downarrow$ & RMSE$\downarrow$
     & LPIPS$\downarrow$ & RMSE$\downarrow$ \\
    \midrule
    \multicolumn{9}{c}{\it Short-range consistency} \\
    \midrule
    %StylizedNeRF ~\citeyear{huang2022stylizednerf} 
    %& 0.071 & 0.056 & 0.037 & 0.029 & 0.043 & 0.034 & 0.111 & 0.103 \\
    \rowcolor[HTML]{E1F2FB}
    StyleGaussian ~\citeyear{liu2024stylegaussian} 
    & 0.033 & 0.038 & 0.031 & 0.034 & 0.038 & 0.037 & 0.069 & 0.061 \\
    \rowcolor[HTML]{F1F9F9}
    G-Style ~\citeyear{kovacs2024gstyle} 
    & 0.042 & 0.052 & 0.032 & 0.035 & 0.038 & 0.034 & 0.066 & 0.070 \\
    \rowcolor[HTML]{F1F9F9}
    StylizedGS\tnote{*} ~\citeyear{zhang2024stylizedgs} 
    & \bftab0.016 & \bftab0.023 & \bftab0.013 & \bftab0.019 & \bftab0.017 & \bftab0.020 & \ul{0.056} & \bftab0.041 \\
    \rowcolor[HTML]{F1F9F9}
    SGSST ~\citeyear{galerne2025sgsst} 
    & 0.038 & 0.047 & 0.039 & 0.047 & 0.044 & 0.049 & 0.084 & 0.090 \\
    %Styl3R~\citeyear{wang2025styl3rinstant3dstylized}
    %& 0.067 & 0.042 & 0.061 & 0.036 & 0.066 & 0.040 & 0.105 & 0.067 \\
    \rowcolor[HTML]{F5EFFF}
    Styl3R~\citeyear{wang2025styl3rinstant3dstylized}
    & -- & -- & 0.061 & 0.036 & 0.066 & 0.040 & 0.105 & 0.067 \\
    \midrule
    \rowcolor[HTML]{F5EFFF}
    \textbf{\textit{Stylos}} (ours) 
    & \ul{0.030} & \ul{0.026} & \ul{0.028} & \ul{0.021} & \ul{0.035} & \ul{0.024} & \bftab0.047 & \ul{0.044} \\
    %\rowcolor{lightgray}
    %\textbf{\textit{Stylos}} (ours new) 
    %& -- & -- & -- & -- & -- & -- & -- & -- \\
    \midrule
    \multicolumn{9}{c}{\it Long-range consistency} \\
    \midrule
    %StylizedNeRF ~\citeyear{huang2022stylizednerf} 
    %& 0.086 & 0.066 & 0.071 & 0.080 & 0.068 & \bftab0.054 & \ul{0.109} & \bftab0.100 \\
    \rowcolor[HTML]{E1F2FB}
    StyleGaussian ~\citeyear{liu2024stylegaussian} 
    & 0.067 & 0.072 & 0.086 & 0.077 & 0.091 & 0.091 & 0.177 & \ul{0.141} \\
    \rowcolor[HTML]{F1F9F9}
    G-Style ~\citeyear{kovacs2024gstyle} 
    & 0.098 & 0.120 & 0.095 & 0.093 & 0.104 & 0.095 & 0.180 & 0.175 \\
    \rowcolor[HTML]{F1F9F9}
    StylizedGS\tnote{*} ~\citeyear{zhang2024stylizedgs} 
    & \bftab0.040 & \ul{0.065} & \bftab0.049 & \bftab0.064 & \bftab0.065 & \ul{0.086} & \bftab0.100 & 0.202 \\
    \rowcolor[HTML]{F1F9F9}
    SGSST ~\citeyear{galerne2025sgsst} 
    & 0.087 & 0.108 & 0.119 & 0.120 & 0.130 & 0.128 & 0.221 & 0.222 \\
    %Styl3R ~\citeyear{wang2025styl3rinstant3dstylized} 
    %& 0.107 & 0.108 & 0.116 & 0.100 & 0.147 & 0.143 & 0.146 & 0.145 \\
    \rowcolor[HTML]{F5EFFF}
    Styl3R ~\citeyear{wang2025styl3rinstant3dstylized} 
    & -- & -- & 0.116 & 0.100 & 0.147 & 0.143 & 0.146 & 0.145 \\
    % \rowcolor{lightgray}
    \midrule
    \rowcolor[HTML]{F5EFFF}
    \textbf{\textit{Stylos}} (ours) 
    & \ul{0.051} & \bftab0.056 & \ul{0.074} & \ul{0.069} & \ul{0.083} & \textbf{0.082} & \ul{0.139} & \bftab0.134 \\
    %\rowcolor{lightgray}
    %\textbf{\textit{Stylos}} (ours new) 
    %& -- & -- & -- & -- & -- & -- & -- & -- \\
    \bottomrule
  \end{tabular}
  \begin{tablenotes}
  \footnotesize
  \item[*] For StylizedGS, cases with \textit{severe color smearing} are excluded when evaluating consistency and ArtScore. Refer to https://github.com/HanzhouLiu/Stylos for reproduced results and evaluation methods.
  \end{tablenotes}
  \end{threeparttable}
  \label{tab:consistency}
\end{table}

